AEON: Adaptive Estimation of Instance-Dependent In-Distribution and Out-of-Distribution Label Noise for Robust Learning

Robust training with noisy labels is a critical challenge in image classification, offering the potential to reduce reliance on costly clean-label datasets. Real-world datasets often contain a mix of in-distribution (ID) and out-of-distribution (OOD) instance-dependent label noise, a challenge that is rarely addressed simultaneously by existing methods and is further compounded by the lack of comprehensive benchmarking datasets. Furthermore, even though current noisy-label learning approaches attempt to find noisy-label samples during training, these methods do not aim to estimate ID and OOD noise rates to promote their effectiveness in the selection of such noisy-label samples, and they are often represented by inefficient multi-stage learning algorithms. We propose the Adaptive Estimation of Instance-Dependent In-Distribution and Out-of-Distribution Label Noise (AEON) approach to address these research gaps. AEON is an efficient one-stage noisy-label learning methodology that dynamically estimates instance-dependent ID and OOD label noise rates to enhance robustness to complex noise settings. Additionally, we introduce a new benchmark reflecting real-world ID and OOD noise scenarios. Experiments demonstrate that AEON achieves state-of-the-art performance on both synthetic and real-world datasets

==> docs/6277259b-7dca-4e1d-ac36-bef451a01c41 <==
{"id":"r0.8592777398151833","lines":[{"id":"n0.2784732834214758","blocks":[],"style":{"align":"center"}},{"blocks":[],"id":"n0.13757949756339016"},{"blocks":[],"style":{"align":"center"},"id":"n0.20742028319942718"},{"blocks":[],"id":"n0.8282144973723045"},{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de784421815272001":{"id":"de784421815272001","lines":[{"blocks":[{"id":"n0.4086868431472226","text":"DOGS","style":{"isBold":true}}],"id":"n0.22718562130935616"}],"shape":{"data":{"p":{"x":49.189424364123184,"y":143.23150565709312},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7925887254797019":{"id":"de7925887254797019","lines":[{"id":"n0.6720073953361116","blocks":[{"id":"n0.8059885967627536","text":"CATS","style":{"isBold":true}}]}],"shape":{"data":{"p":{"x":148.495983935743,"y":143.83434870902238},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de33937106756927005":{"id":"de33937106756927005","lines":[{"blocks":[{"text":"CATS","style":{"isBold":true},"id":"n0.46546521407423147"}],"id":"n0.32857272759520706"}],"shape":{"data":{"p":{"x":49.92570281124499,"y":259.5802146794314},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6887015639086216":{"id":"de6887015639086216","lines":[{"blocks":[{"text":"DOGS","style":{"isBold":true},"id":"n0.2540277597830962"}],"id":"n0.94012107319956"}],"shape":{"data":{"p":{"x":144.60040160642575,"y":258.9773716275022},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de6265300194773114":{"id":"de6265300194773114","lines":[{"blocks":[{"text":"CATS","style":{"isBold":true},"id":"n0.4344503767766532"}],"id":"n0.8474145525785008"}],"shape":{"data":{"p":{"x":147.8641231593039,"y":381.95735422106185},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8626755972977136":{"id":"de8626755972977136","lines":[{"blocks":[{"text":"DOGS","style":{"isBold":true},"id":"n0.3532655051845879"}],"id":"n0.6783919110000816"}],"shape":{"data":{"p":{"x":61.194779116465895,"y":381.3545111691326},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de1667098316447051":{"id":"de1667098316447051","lines":[{"id":"n0.23679964223957017","blocks":[{"id":"n0.9957058120423361","text":"Clean-Set","style":{"isBold":true}}]}],"shape":{"data":{"p":{"x":83.28915662650606,"y":53.70931244560488},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4036225697807241":{"id":"de4036225697807241","lines":[{"blocks":[{"text":"Closed-Set","style":{"isBold":true},"id":"n0.8668571862089922"}],"id":"n0.6972506115947765"}],"shape":{"data":{"p":{"x":80.52677376171353,"y":168.85233536408472},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8557666737420511":{"id":"de8557666737420511","lines":[{"blocks":[{"text":"Open-Set","id":"n0.26364740527926633","style":{"isBold":true}}],"id":"n0.201135762003551"}],"shape":{"data":{"p":{"x":89.6599732262383,"y":291.2294749057151},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de4647841738017484":{"id":"de4647841738017484","lines":[{"id":"n0.317015050529843","blocks":[{"id":"n0.002243027946460252","text":"𝛾","style":{"mathType":"\\mathbf"}},{"id":"n0.9881410590612076","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.3228808632092153","lines":[{"id":"n0.2249472848069165","blocks":[{"id":"n0.7520974113698669","text":"in"}]}]}},"style":{"mathType":"\\mathbf"}}]}],"shape":{"data":{"p":{"x":546,"y":140}},"anchor":"left-top","style":{"fillColor":[245,166,35,1]}},"isMathDisplayMode":true,"isInGroup":true},"de8442248373843018":{"id":"de8442248373843018","lines":[{"id":"n0.3794779090901039","blocks":[{"id":"n0.016476944364607782","text":"Supervised","style":{"isBold":true}}]}],"shape":{"data":{"p":{"x":999.6379310344828,"y":147},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de008246533557802138":{"id":"de008246533557802138","lines":[{"blocks":[{"text":"Unsupervised","id":"n0.13776105829121077","style":{"isBold":true}}],"id":"n0.044218114389454666"}],"shape":{"data":{"p":{"x":991,"y":202},"rotation":0},"anchor":"left-top","style":{"fillColor":[139,87,42,0.1]}},"isTextMode":true,"isInGroup":true},"de506560423209403":{"id":"de506560423209403","lines":[{"blocks":[{"id":"n0.6265532281967661","text":"Contrastive","style":{"isBold":true}}],"id":"n0.5811856116214658"}],"shape":{"data":{"p":{"x":1002,"y":257},"rotation":0},"anchor":"left-top","style":{"fillColor":[139,87,42,0.1]}},"isTextMode":true,"isInGroup":true},"de2398185149548706":{"id":"de2398185149548706","lines":[{"id":"n0.22549257477740214","blocks":[{"id":"n0.23656965164134225","text":"D = ","style":{"mathType":"\\mathbf"}},{"id":"n0.5780854048098323","type":"single","text":"{","style":{"mathType":"\\mathbf"}},{"id":"n0.29486678212548245","text":"\\hat","type":"composite","elements":{"value":{"id":"n0.6875650519271814","lines":[{"id":"n0.13717697206876478","blocks":[{"id":"n0.2241014359537341","text":"X"}]}]}},"style":{"mathType":"\\mathbf"}},{"id":"n0.5558556386662121","text":", ","style":{"mathType":"\\mathbf"}},{"id":"n0.8961281101600986","text":"\\hat","type":"composite","elements":{"value":{"id":"n0.7994860270494852","lines":[{"id":"n0.7486024603272687","blocks":[{"id":"n0.06702583477861235","text":"Y"}]}]}},"style":{"mathType":"\\mathbf"}},{"id":"n0.7647832997781878","type":"single","text":"}","style":{"mathType":"\\mathbf"}}]}],"shape":{"data":{"p":{"x":64.66666666666667,"y":21}},"anchor":"left-top"},"isMathDisplayMode":true,"isInGroup":true},"de8409841721712077":{"id":"de8409841721712077","lines":[{"id":"n0.7140190339391934","blocks":[{"id":"n0.12978842609876784","text":"D","style":{"mathType":"\\mathbf"}}]}],"shape":{"data":{"p":{"x":244,"y":194}},"anchor":"left-top"},"isMathDisplayMode":true,"isInGroup":true},"de5193583289417196":{"id":"de5193583289417196","lines":[{"id":"n0.5930649211639134","blocks":[{"id":"n0.6826749761800728","text":"f"},{"id":"n0.07836210697890689","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.1973364313529513","lines":[{"id":"n0.08064081621677999","blocks":[{"id":"n0.7007409587512117","text":"𝜃"}]}]}}}]}],"shape":{"data":{"p":{"x":294,"y":205}},"anchor":"left-top","settings":{"fontSize":"\\Large"}},"isMathDisplayMode":true,"isInGroup":true},"de36551762287250344":{"id":"de36551762287250344","lines":[{"blocks":[{"text":"f","id":"n0.9693873444886318"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"𝜃","id":"n0.5517475424948368"}],"id":"n0.8049894966785267"}],"id":"n0.3472341428440482"}},"id":"n0.2465960532084177"}],"id":"n0.19097435098045068"}],"shape":{"data":{"p":{"x":396,"y":62}},"anchor":"left-top","settings":{"fontSize":"\\normalsize"}},"isMathDisplayMode":true,"isInGroup":true},"de7385129204075771":{"id":"de7385129204075771","lines":[{"blocks":[{"text":"f","id":"n0.17133423222379363"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"𝜃","id":"n0.09886884582449218"}],"id":"n0.2778694341554415"}],"id":"n0.855310621017511"}},"id":"n0.6394101765931051"}],"id":"n0.04407447722927893"}],"shape":{"data":{"p":{"x":393,"y":325}},"anchor":"left-top","settings":{"fontSize":"\\normalsize"}},"isMathDisplayMode":true,"isInGroup":true},"de7179193903364058":{"id":"de7179193903364058","lines":[{"id":"n0.20205173932349552","blocks":[{"id":"n0.7648963627367806","text":"Energy-Scores","style":{"isBold":true}}]}],"shape":{"data":{"p":{"x":438,"y":80}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8341430273373942":{"id":"de8341430273373942","lines":[{"blocks":[{"id":"n0.044370934135517626","text":"Loss-values","style":{"isBold":true}}],"id":"n0.18776184862733958"}],"shape":{"data":{"p":{"x":449,"y":345}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de9185186072278175":{"id":"de9185186072278175","lines":[{"blocks":[{"text":"𝛾","style":{"mathType":"\\mathbf"},"id":"n0.3964201554891498"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.07620750675319399","text":"out"}],"id":"n0.9966099325240185"}],"id":"n0.8280717938164819"}},"style":{"mathType":"\\mathbf"},"id":"n0.8632585306069149"}],"id":"n0.4181549337393382"}],"shape":{"data":{"p":{"x":551,"y":268}},"anchor":"left-top"},"isMathDisplayMode":true,"isInGroup":true},"de7326708460425577":{"id":"de7326708460425577","lines":[{"id":"n0.1923050163967739","blocks":[{"id":"n0.2889108764804027","text":"𝜂","style":{"mathType":"\\mathbf"}},{"id":"n0.41865489886699603","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.21144013434345377","lines":[{"id":"n0.3246886795730428","blocks":[{"id":"n0.8392641176941018","text":"i"}]}]}},"style":{"mathType":"\\mathbf"}},{"id":"n0.9026033684162171","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.003375406702789574","lines":[{"id":"n0.13163993065133295","blocks":[{"id":"n0.8120796438855942","text":"n"}]}]}},"style":{"mathType":"\\mathbf"}}]}],"shape":{"data":{"p":{"x":808,"y":263}},"anchor":"left-top"},"isMathDisplayMode":true,"isInGroup":true},"de08217707543734942":{"id":"de08217707543734942","lines":[{"blocks":[{"text":"𝜂","style":{"mathType":"\\mathbf"},"id":"n0.7728906549703505"},{"id":"n0.0872572177850397","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.012690971071541046","lines":[{"id":"n0.8170690258315227","blocks":[{"id":"n0.8846943604315007","text":"out"}]}]}},"style":{}}],"id":"n0.7411586509217203"}],"shape":{"data":{"p":{"x":799,"y":85}},"anchor":"left-top"},"isMathDisplayMode":true,"isInGroup":true},"de14157623548794507":{"id":"de14157623548794507","lines":[{"id":"n0.3168108497680535","blocks":[{"id":"n0.5688522361845445","text":"w"},{"id":"n0.09694842473549503","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.439776756521602","lines":[{"id":"n0.9177536380984335","blocks":[{"id":"n0.18075020952540477","text":"out"}]}]}}}]}],"shape":{"data":{"p":{"x":845,"y":95}},"anchor":"left-top","settings":{"fontSize":"\\LARGE"}},"isMathDisplayMode":true,"isInGroup":true},"de7501474550197778":{"id":"de7501474550197778","lines":[{"blocks":[{"text":"w","id":"n0.11680633612181923"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9944866173324463","text":"in"}],"id":"n0.6940233480927769"}],"id":"n0.23634607808072516"}},"id":"n0.6652696780677565"}],"id":"n0.9938217744990634"}],"shape":{"data":{"p":{"x":854,"y":270}},"anchor":"left-top","settings":{"fontSize":"\\LARGE"}},"isMathDisplayMode":true,"isInGroup":true},"de07498895703967312":{"id":"de07498895703967312","lines":[{"id":"n0.5216191503548335","blocks":[{"id":"n0.5018649169303193","text":"Noisy Label Training","style":{"isBold":true}}]}],"shape":{"data":{"p":{"x":969,"y":94}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7721070156321141":{"id":"de7721070156321141","lines":[{"id":"n0.06789689210621774","blocks":[{"id":"n0.13032348874924704","text":"sample ","style":{"isBold":true}}]},{"id":"n0.5986594034312596","blocks":[{"text":"masking","id":"n0.46339870553943197","style":{"isBold":true}}],"style":null}],"shape":{"data":{"p":{"x":838,"y":50}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de7956490652676713":{"id":"de7956490652676713","lines":[{"blocks":[{"text":"sample ","style":{"isBold":true},"id":"n0.6376222302187913"}],"id":"n0.7625535998346042"},{"blocks":[{"text":"masking","style":{"isBold":true},"id":"n0.352839657844243"}],"style":null,"id":"n0.16991468616980887"}],"shape":{"data":{"p":{"x":843,"y":324}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de26081267593690227":{"id":"de26081267593690227","lines":[{"id":"n0.1434505891307123","blocks":[{"id":"n0.2649612698685908","text":"Open-set Sigmoid Soft Masking","style":{"isBold":true,"fontSize":"\\large"}}]}],"shape":{"data":{"p":{"x":512,"y":19}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de13400908333478379":{"id":"de13400908333478379","lines":[{"blocks":[{"text":"Closed-set Sigmoid Soft Masking","id":"n0.21872481002103417","style":{"isBold":true,"fontSize":"\\large"}}],"id":"n0.40743899601059175"}],"shape":{"data":{"p":{"x":509,"y":399}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de14448633998070926":{"id":"de14448633998070926","lines":[{"blocks":[{"id":"n0.2783483972718166","text":"Warmup","style":{"isBold":true}}],"id":"n0.6432534468869011"}],"shape":{"data":{"p":{"x":278.6666666666667,"y":261.3333333333333}},"anchor":"left-top"},"isTextMode":true,"isInGroup":true},"de8862976222601386":{"id":"de8862976222601386","lines":[{"id":"n0.9199461818108496","blocks":[{"id":"n0.9166744329277965","text":"Learnables","style":{"isBold":true}}]}],"shape":{"data":{"p":{"x":1056,"y":-3.882772360483308},"rotation":0},"anchor":"left-top"},"isTextMode":true,"isInGroup":true}},"connections":[],"intersections":{"id":"di09026383366009993","items":[],"style":{}},"shapes":[{"id":"dg35846218671995","entities":[{"id":"dp9929472174264573","type":"doc-rounded-rect","data":{"p1":{"x":370.5,"y":232},"p2":{"x":916,"y":389}},"style":{"fillColor":[255,0,0,0.1]}},{"id":"dp714803500292295","type":"doc-rounded-rect","data":{"p1":{"x":369.5,"y":50},"p2":{"x":918,"y":187}},"style":{"fillColor":[0,0,255,0.05]}},{"id":"dg6837568170269519","entities":[{"id":"dg2693894476408103","entities":[{"id":"dg7059289805805817","entities":[{"id":"dp036634938853897125","type":"image","data":{"p1":{"x":42.25435073627848,"y":318.50623730780393},"p2":{"x":127.5555555555556,"y":386.0246591238759},"url":"data-resources/43b4c102-8106-4457-874a-9720e8febd6a"}},{"id":"dp0534459982184321","type":"image","data":{"p1":{"x":130.39892904953155,"y":314.8891789962286},"p2":{"x":212.22489959839362,"y":380.59907165651293},"url":"data-resources/a851a816-23cb-4db4-9172-a6a70e7223b3"}},{"id":"dp08602763097520238","type":"doc-rounded-rect","data":{"p1":{"x":40.35876840696122,"y":312.1161009573542},"p2":{"x":207.17001338688087,"y":400.73402959094864}},"style":{"fillColor":[74,144,226,0.1]}},{"id":"dl5228875844763949","linkedId":"de6265300194773114"},{"id":"dl46431639039457084","linkedId":"de8626755972977136"}],"data":{"rotation":0}},{"id":"dl9708126295069972","linkedId":"de8557666737420511"}],"data":{"rotation":0}},{"id":"dg8122192073718124","entities":[{"id":"dg447126185671088","entities":[{"id":"dg26709674553925633","entities":[{"id":"dp6748860182322836","type":"image","data":{"p1":{"x":112.70682730923697,"y":72.39556135770235},"p2":{"x":219.33333333333337,"y":150.16231505657095},"url":"data-resources/1a389895-78ba-401b-af5b-7b4096ceccb4"}},{"id":"dl563882584903499","linkedId":"de7925887254797019"}],"data":{"rotation":0}},{"id":"dg32693949919633636","entities":[{"id":"dp6491890221222434","type":"image","data":{"p1":{"x":29.301204819277128,"y":71.34058601682621},"p2":{"x":120.76305220883538,"y":145.0381491151726},"url":"data-resources/a4e59c8a-f7f2-4473-a3fd-c4147dea5bcb"}},{"id":"dl894572680808992","linkedId":"de784421815272001"}],"data":{"rotation":0}},{"id":"dp29425053136621715","type":"doc-rounded-rect","data":{"p1":{"x":36.567603748326675,"y":73.14911517261388},"p2":{"x":210.32931726907634,"y":161.76704380620833}},"style":{"fillColor":[184,233,134,0.1]}}],"data":{"rotation":0}},{"id":"dl7875920018490135","linkedId":"de1667098316447051"}],"data":{"rotation":0}},{"id":"dg42144738182936403","entities":[{"id":"dg7035473620380412","entities":[{"id":"dp38493097207842175","type":"image","data":{"p1":{"x":132.61044176706832,"y":186.48360893530605},"p2":{"x":210.3293172690763,"y":262.44183347838697},"url":"data-resources/cc0013e2-5ec2-4099-9bd6-cdb0eced9b78"}},{"id":"dp09624536424228602","type":"image","data":{"p1":{"x":22.666666666666686,"y":187.3878735131999},"p2":{"x":118.7095046854083,"y":263.6475195822454},"url":"data-resources/ce7bf60d-3aa4-4cf6-89c7-2df57e88f670"}},{"id":"dp5799465097338554","type":"doc-rounded-rect","data":{"p1":{"x":36.56760374832665,"y":191.54749057151145},"p2":{"x":210.3293172690763,"y":280.1654192051059}},"style":{"fillColor":[255,0,0,0.1]}},{"id":"dl014007913519534121","linkedId":"de33937106756927005"},{"id":"dl991517699347187","linkedId":"de6887015639086216"}],"data":{"rotation":0}},{"id":"dl32105988332651036","linkedId":"de4036225697807241"}],"data":{"rotation":0}}],"data":{}},{"id":"dp9650909821062645","type":"doc-rounded-rect","data":{"p1":{"x":22.666666666666657,"y":52.333333333333336},"p2":{"x":222.66666666666663,"y":413.6666666666667}}},{"id":"da45538594413412503","data":[{"x":222,"y":222},{"x":289,"y":222}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"dp06393606395115703","type":"flow-manual-operation","data":{"p1":{"x":275,"y":202},"p2":{"x":345,"y":242},"rotation":271.25},"style":{"fillColor":[245,166,35,1]}},{"id":"da3019881441816443","data":[{"x":334.5,"y":222.75},{"x":383,"y":223.75}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"da2213346906083058","data":[{"x":383,"y":92},{"x":383,"y":355.5}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da1502368792319959","data":[{"x":383,"y":92},{"x":431.5,"y":93}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"da9297382761139088","data":[{"x":383,"y":355.5},{"x":426.5,"y":357}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"dp16412852818490853","type":"doc-rounded-rect","data":{"p1":{"x":432,"y":72},"p2":{"x":553,"y":112}},"style":{"fillColor":[74,144,226,0.1]}},{"id":"dp7737040529429617","type":"doc-rounded-rect","data":{"p1":{"x":430,"y":336},"p2":{"x":556,"y":376}},"style":{"fillColor":[255,0,0,0.1]}},{"id":"dg6340960628608867","entities":[{"id":"da9995165647577686","data":[{"x":596,"y":92},{"x":596,"y":132}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da22296253955983714","data":[{"x":596,"y":132},{"x":619,"y":132}],"head":"fh>","tail":"no","shaft":"-","mVer":1}],"data":{}},{"id":"da19302241000103648","data":[{"x":555,"y":92},{"x":596,"y":92}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da810685439363916","data":[{"x":596,"y":323},{"x":596,"y":356}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6156063543037473","data":[{"x":596,"y":323},{"x":624,"y":323}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"da726452698890288","data":[{"x":557,"y":356},{"x":596,"y":356}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp08604171238843183","type":"image","data":{"p1":{"x":623,"y":65},"p2":{"x":792,"y":179},"url":"data-resources/65b5e33e-efda-4f4f-986c-722de945ba1e"}},{"id":"dg048412160764108814","entities":[{"id":"dp04477356116735076","type":"circle","data":{"p1":{"x":533,"y":129},"p2":{"x":583,"y":179}},"style":{"fillColor":[245,166,35,1]}},{"id":"dl8644635233924469","linkedId":"de4647841738017484"}]},{"id":"dp8051061427559867","type":"circle","data":{"p1":{"x":541,"y":257},"p2":{"x":591,"y":307}},"style":{"fillColor":[245,166,35,1]}},{"id":"da8825968669524231","data":[{"x":583,"y":154},{"x":621,"y":154}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"da5473167467686535","data":[{"x":591,"y":282},{"x":629,"y":282}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"dp48704195826545016","type":"image","data":{"p1":{"x":632,"y":241},"p2":{"x":801,"y":355},"url":"data-resources/1e45fb2c-f93f-4bba-987a-5b47147eac9a"}},{"id":"da7750141875969183","data":[{"x":802,"y":297},{"x":844,"y":298}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"da40320072972446486","data":[{"x":794,"y":122},{"x":836,"y":122}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"dp4980325541112254","type":"doc-rounded-rect","data":{"p1":{"x":841,"y":100},"p2":{"x":908,"y":140}},"style":{"fillColor":[74,144,226,0.1]}},{"id":"dp7409333763260224","type":"doc-rounded-rect","data":{"p1":{"x":848,"y":276},"p2":{"x":910,"y":316}},"style":{"fillColor":[255,0,0,0.1]}},{"id":"da05192110668589689","data":[{"x":912,"y":120},{"x":930,"y":120}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9412524998529657","data":[{"x":930,"y":120},{"x":928.5,"y":301}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3502231408330707","data":[{"x":912,"y":301},{"x":928.5,"y":301}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da85117023472375","data":[{"x":930,"y":213},{"x":972,"y":214}],"head":"fh>","tail":"no","shaft":"-","mVer":1},{"id":"dg40565155799950814","entities":[{"id":"dp3816600617085528","type":"doc-rounded-rect","data":{"p1":{"x":974,"y":121},"p2":{"x":1113,"y":308}},"style":{"fillColor":[189,16,224,0.1]}},{"id":"dg9435210906000839","entities":[{"id":"dp8388277910239788","type":"doc-rounded-rect","data":{"p1":{"x":986,"y":139},"p2":{"x":1098,"y":179}},"style":{"fillColor":[139,87,42,0.1]}},{"id":"dl9872093135996776","linkedId":"de8442248373843018"}]},{"id":"dg01682467220274031","entities":[{"id":"dp4007724852204966","type":"doc-rounded-rect","data":{"p1":{"x":988,"y":195},"p2":{"x":1100,"y":235}},"style":{"fillColor":[139,87,42,0.1]}},{"id":"dl6746647098108731","linkedId":"de008246533557802138"}]},{"id":"dg028865211948478242","entities":[{"id":"dp8263433966973108","type":"doc-rounded-rect","data":{"p1":{"x":988,"y":249},"p2":{"x":1100,"y":289}},"style":{"fillColor":[139,87,42,0.1]}},{"id":"dl6169237865984956","linkedId":"de506560423209403"}]}]},{"id":"dl25444737428927056","linkedId":"de2398185149548706"},{"id":"dl8782158517506953","linkedId":"de8409841721712077"},{"id":"dl33475815703299827","linkedId":"de5193583289417196"},{"id":"dl607363722338264","linkedId":"de36551762287250344"},{"id":"dl28434115928479264","linkedId":"de7385129204075771"},{"id":"dl07081708386224572","linkedId":"de7179193903364058"},{"id":"dl012460631251480558","linkedId":"de8341430273373942"},{"id":"dl12266636568273004","linkedId":"de9185186072278175"},{"id":"dl25286690747522456","linkedId":"de7326708460425577"},{"id":"dl46967710921330097","linkedId":"de08217707543734942"},{"id":"dl6859733569959836","linkedId":"de14157623548794507"},{"id":"dl8412638907216816","linkedId":"de7501474550197778"},{"id":"dl265722660698394","linkedId":"de07498895703967312"},{"id":"dl28021929641419097","linkedId":"de7721070156321141"},{"id":"dl08112193247959132","linkedId":"de7956490652676713"},{"id":"dl13451784155029745","linkedId":"de26081267593690227"},{"id":"dl583810882582958","linkedId":"de13400908333478379"},{"id":"dl04236695066304774","linkedId":"de14448633998070926"}]},{"id":"dg4133824959038228","entities":[{"id":"dp21630119627333144","type":"ellipse","data":{"p1":{"x":1101.4819277108434,"y":25.390758798388966},"p2":{"x":1126,"y":50.78151759677793}},"style":{"fillColor":[245,166,35,1]}},{"id":"dp5260488206684586","type":"flow-manual-operation","data":{"p1":{"x":1064.381574307653,"y":28.898801778182282},"p2":{"x":1099.9953395860275,"y":46.902675149315954},"rotation":271.14,"skewX":-0.23},"style":{"fillColor":[245,166,35,1]}},{"id":"dl23983470777370086","linkedId":"de8862976222601386"}]}],"settings":{"grid":true,"diagramHeight":430,"gridSize":44,"gridBold":false},"id":"n0.003983592314337869"}],"id":"n0.8071057420812084"}],"pageSettings":{"pageSize":{"width":1182,"sizeUnit":"px"}},"___version":2,"version":2,"av":1856,"delayRenderCache":{"av":1856,"map":{}}}

==> preamble.tex <==
\newcommand{\gustavo}[1]{\textcolor{brown}{Gustavo: #1}}
\newcommand{\cuong}[1]{\textcolor{magenta}{Cuong: #1}}
\newcommand{\rafa}[1]{\textcolor{ForestGreen}{Rafa: #1}}
\newcommand{\toan}[1]{\textcolor{Cyan}{Toan: #1}}
%my command
\newcommand{\arpit}[1]{\textcolor{orange}{Arpit: #1}}
\usepackage[dvipsnames]{xcolor}
\usepackage[table]{xcolor}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric} % Load the shapes.geometric library
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usetikzlibrary{pgfplots.groupplots}
\pgfplotsset{compat=1.15}
\usetikzlibrary{arrows.meta}
\pgfplotsset{compat=newest}
\usepackage{dirtytalk}
\usepackage{nicefrac} 
\usepackage{algorithm}
\usepackage{colortbl}
\usepackage{algpseudocodex}
\usepackage{multirow}
\usepackage[normalem]{ulem}
\usepackage{booktabs}
% \usepackage[backend=bibtex,style=numeric]{biblatex}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{pifont}
\newcommand{\xmark}{\text{\sffamily X}}


\definecolor{C0}{HTML}{1f77b4}
\definecolor{C1}{HTML}{ff7f0e}

\usepackage{adjustbox}

\newcommand{\customeqref}[1]{equation~(\ref{#1})}
\newcommand{\withdagger}[1]{#1\(^{\dagger}\)}

\usepackage{graphicx} % Include the graphicx package for including graphics
\usepackage{subcaption} % Include the subcaption package for subfigures
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert} % Defines the \norm command
\newcommand{\frobnorm}[1]{\lVert#1\rVert_F}
\usepackage{physics}

\newcommand{\passLine}{\tikz[baseline=-0.5ex]{\draw[dash dot, BrickRed, line width=1pt] (0,0) -- (0.5,0);}}
\newcommand{\mentorNetLine}{\tikz[baseline=-0.5ex]{\draw[dashed, BurntOrange, line width=1pt] (0,0) -- (0.5,0);}}
\newcommand{\fineLine}{\tikz[baseline=-0.5ex]{\draw[solid, MidnightBlue, line width=1pt] (0,0) -- (0.5,0);}}


% Define robust commands
\DeclareRobustCommand{\passLine}{
  \tikz[baseline=-0.5ex]{
    \draw[dash dot, BrickRed, line width=1pt] (0,0) -- (0.5,0);
  }
}

\DeclareRobustCommand{\mentorNetLine}{
  \tikz[baseline=-0.5ex]{
    \draw[dashed, BurntOrange, line width=1pt] (0,0) -- (0.5,0);
  }
}

\DeclareRobustCommand{\fineLine}{
  \tikz[baseline=-0.5ex]{
    \draw[solid, MidnightBlue, line width=1pt] (0,0) -- (0.5,0);
  }
}
\DeclareRobustCommand{\solidBlue}{
  \tikz[baseline=-0.5ex]{
    \draw[solid, MidnightBlue, line width=1pt] (0,0) -- (0.5,0);
  }
}

\DeclareRobustCommand{\dashedYellow}{
  \tikz[baseline=-0.5ex]{
    \draw[dashed, BurntOrange, line width=1pt] (0,0) -- (0.5,0);
  }
}
% Define robust command for clean samples (Thick solid line with * markers)
% Define robust command for clean samples (solid blue line)
% \DeclareRobustCommand{\cleanLine}{
%   \tikz[baseline=0.5ex]{
%     \draw[mark=*, mark size=0.5pt, thick, solid, MidnightBlue!70] (0,0) -- (0.3,0);
%     \node[MidnightBlue!70, fill=MidnightBlue!70, circle, inner sep=0.5pt] at (0.15,0) {*};
%   }
% }

\DeclareRobustCommand{\cleanLine}{
  \tikz[baseline=-0.5ex]{
    \draw[thick, solid, MidnightBlue!70] (0,0) -- (0.6,0);
     \node[circle, fill=MidnightBlue, inner sep=1.5pt, minimum size=3pt] at (0.3,0) {};
  }
}

% Define robust command for noisy samples (thick solid line with • marker)
\DeclareRobustCommand{\noisyLine}{
  \tikz[baseline=-0.5ex]{
    \draw[thick, solid, BurntOrange!70] (0,0) -- (0.6,0);
    \node[diamond, fill=BurntOrange!70, inner sep=1.5pt, minimum size=3pt] at (0.3,0) {};
  }
}
\usepackage{amssymb}
\newcommand{\checkmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
